Scaling Empowered Agents

Empowerment measures the capacity of an agent to actively control its environment. In this work, we explain the connection between skill learning and empowerment. While skill learning is not empowerment, we introduce a simple scalable recipe for empowerment maximization: empowerment corresponds to the number of executable skills from a state, so maximizing empowerment corresponds to reaching states that are good starting points for many skills. Our recipe applies to arbitrary underlying skill learning methods. Whereas most prior work on empowerment looks at tabular settings, this recipe enables us to study empowerment at a scale where we can realize theoretically-predicted but empirically-elusive properties of empowerment (e.g., gathering resources, environment modification, survival). Experiments show that empowerment maximization unlocks interesting emergent properties, such as building a house in Crafter. Website and code at \href{https://empowerment-geometry.github.io/scaling-empowerment/}{this https url}.

==> definitions.tex <==
\newglossaryentry{pi_mathrmeff}{%
	sort={pieff},
	name={\ensuremath{\pi_{\mathrm{eff}}}},
	description={an effective empowerment maximizing policy}
}

\newglossaryentry{pi_mathrmpot}{%
	sort={pipot},
	name={\ensuremath{\pi_{\mathrm{pot}}}},
	description={a potential empowerment maximizing policy}
}

\newglossaryentry{ge_mathrmeff}{%
	sort={geeff},
	name={\ensuremath{\gE_{\mathrm{eff}}}},
	description={the effective empowerment as a function of the policy}
}

\newglossaryentry{ge_mathrmpot}{%
	sort={gepot},
	name={\ensuremath{\gE_{\mathrm{pot}}}},
	description={the potential empowerment as a function of the state}
}

\newglossaryentry{gaussian_width}{%
	sort={gaussian width},
	name={Gaussian width},
	description={$w(\Theta)\triangleq\E\sup_{\theta\in\Theta}\langle\theta,Z\rangle$, $Z\sim\cN(0,I_d)$, for $\Theta\subset\mathbb{R}^d$ \citep[Eq.~(27.19)]{polyanskiy2025information}}
}


\newacronym{mdp}{MDP}{Markov decision process}
\newacronym{mi}{MI}{mutual information}
\newacronym[type=main,first={Metric-aware Abstraction (METRA)},description={Metric-aware Abstraction~\citep{park2024metra}}]{metra}{METRA}{Metric-aware Abstraction}

\newacronym[type=main,first={contrastive successor features (CSF)},description={contrastive successor features~\citep{zheng2025misl}}]{csf}{CSF}{contrastive successor features}
\newacronym{dsom}{DSOM}{discounted state occupancy measure}
\newacronym[type=main,first={hindsight experience replay (HER)},description={hindsight experience replay~\citep{andrychowicz2017hindsight}}]{her}{HER}{hindsight experience replay}

\newacronym{ib}{IB}{information bottleneck}
\newacronym{kl}{KL}{Kullback-Leibler}
\newacronym{misl}{MISL}{mutual information skill learning}

\newacronym{rl}{RL}{reinforcement learning}
\newacronym{vib}{VIB}{variational information bottleneck}
\newacronym{usd}{USD}{unsupervised skill discovery}
\newacronym{lqr}{LQR}{linear-quadratic regulator}

\newglossaryentry{vim}{name={VIM},description={variational information maximization~\citep{mohamed2015variational}}}
\newglossaryentry{variationalempowerment}{name={variational empowerment},description={empowerment maximization with a variational bound and learned dynamics~\citep{karl2017unsupervised}}}
\newglossaryentry{latentgce}{name={LatentGCE},description={latent Gaussian-channel empowerment~\citep{zhao2021efficient}}}
\newglossaryentry{vic}{name={VIC},description={variational intrinsic control~\citep{gregor2017variational}}}
\newglossaryentry{infonce}{name={InfoNCE},description={information noise-contrastive estimation~\citep{oord2018representation}}}
\newacronym[description={conditional mutual information}]{cmi}{CMI}{conditional mutual information}
\newacronym[type=main,first={soft actor-critic (SAC)},description={soft actor-critic~\citep{haarnoja2018soft}}]{sac}{SAC}{soft actor-critic}
\newacronym[type=main,first={proximal policy optimization (PPO)},description={proximal policy optimization~\citep{schulman2017proximal}}]{ppo}{PPO}{proximal policy optimization}
\newacronym[type=main,first={parallelized Q-network (PQN)},description={parallelized Q-network~\citep{gallici2025simplifying}}]{pqn}{PQN}{parallelized Q-network}

